Generalized Species Sampling Priors with Latent Beta reinforcements

Many popular Bayesian nonparametric priors can be characterized in terms of exchangeable species sampling sequences. However, in some applications, exchangeability may not be appropriate. We introduce a {novel and probabilistically coherent family of non-exchangeable species sampling sequences characterized by a tractable predictive probability function with weights driven by a sequence of independent Beta random variables. We compare their theoretical clustering properties with those of the Dirichlet Process and the two parameters Poisson-Dirichlet process. The proposed construction provides a complete characterization of the joint process, differently from existing work. We then propose the use of such process as prior distribution in a hierarchical Bayes modeling framework, and we describe a Markov Chain Monte Carlo sampler for posterior inference. We evaluate the performance of the prior and the robustness of the resulting inference in a simulation study, providing a comparison with popular Dirichlet Processes mixtures and Hidden Markov Models. Finally, we develop an application to the detection of chromosomal aberrations in breast cancer by leveraging array CGH data.

==> HMMTable_2_res.tex <==
\begin{center}
\begin{tabular}{|l|cccc|ccc|}
\hline 
\multicolumn{8}{|l|}{\textbf{Data Generating Process: Hidden Semi Markov Model (HSMM) with
4 states and }NegBin$(50,5)$ }\tabularnewline
\hline 
 & \multicolumn{7}{c|}{$\tau=0.25$}\tabularnewline
\hline 
\multicolumn{1}{|l|}{\textbf{Simulation Method}} & \multicolumn{4}{c|}{\textbf{Beta-Gos}} & \multicolumn{3}{c|}{\textbf{HMM}}\tabularnewline
 & \multicolumn{1}{c}{$\alpha_{n}=n;\, \beta_{n}=1$} & \multicolumn{1}{c}{$\alpha_{n}=5;\, \beta_{n}=1$} & \multicolumn{1}{c}{$\alpha_{n}=1;\beta_{n}=1$} & \multicolumn{1}{c|}{$\alpha_{n}=1;\: \beta_{n}=3$} & \multicolumn{1}{c}{3 States} & \multicolumn{1}{c}{4 States} & \multicolumn{1}{c|}{5 States}\tabularnewline
\hline 
\textbf{Number of clusters} &  &  &  &  &  &  & \tabularnewline
~~Ground truth & $4.00$$\pm$$0.00$ & $4.00$$\pm$$0.00$ & $4.00\pm$$0.00$ & $4.00$$\pm$0.00 & 4.00$\pm$0.00 & 4.00$\pm$0.00 & 4.00$\pm$0.00\tabularnewline
~~Estimation & $3.97$$\pm0.70$ & $3.97$$\pm0.71$ & $3.84$$\pm$$0.56$ & $3.74$$\pm$0.50 & 2.99$\pm$0.11 & 3.86$\pm$0.48 & 4.58$\pm$0.93\tabularnewline
\hline 
\textbf{Cluster assignment} &  &  &  &  &  &  & \tabularnewline
~~Accuracy & 0.95$\pm$0.09 & 0.95$\pm$0.08 & 0.95$\pm$0.09 & 0.94$\pm$0.09 & 0.78$\pm$0.10 & 0.87$\pm$0.13 & 0.89$\pm$0.16\tabularnewline
\hline 
 & \multicolumn{7}{c|}{$\tau=0.5$}\tabularnewline
\hline 
\textbf{Number of clusters} & \multicolumn{4}{l|}{} & \multicolumn{3}{c|}{}\tabularnewline
~~Estimation & 3.87$\pm$0.98 & 3.88$\pm$0.97 & 3.59$\pm0.79$ & 3.38$\pm$0.72 & 2.99$\pm$0.13 & 3.87$\pm0.47$ & $4.64$$\pm0.88$\tabularnewline
\textbf{Cluster assignment} &  &  &  &  &  &  & \tabularnewline
~~Accuracy & 0.89$\pm0.13$ & $0.90\pm0.12$ & 0.88$\pm0.13$ & $0.85\pm$0.14 & $0.77\pm0.10$ & 0.85$\pm0.13$ & $0.87\pm0.15$\tabularnewline
\hline 
\end{tabular}
\par\end{center}


